When Choosing Plausible Alternatives, Clever Hans can be Clever

Pretrained language models, such as BERT and RoBERTa, have shown large improvements in the commonsense reasoning benchmark COPA. However, recent work found that many improvements in benchmarks of natural language understanding are not due to models learning the task, but due to their increasing ability to exploit superficial cues, such as tokens that occur more often in the correct answer than the wrong one. Are BERT's and RoBERTa's good performance on COPA also caused by this? We find superficial cues in COPA, as well as evidence that BERT exploits these cues. To remedy this problem, we introduce Balanced COPA, an extension of COPA that does not suffer from easy-to-exploit single token cues. We analyze BERT's and RoBERTa's performance on original and Balanced COPA, finding that BERT relies on superficial cues when they are present, but still achieves comparable performance once they are made ineffective, suggesting that BERT learns the task to a certain degree when forced to. In contrast, RoBERTa does not appear to rely on superficial cues.

==> tables/all_balanced_pairwise_annotation_artifacts.tex <==
\begin{table}[t]
    \centering
    \begin{tabularx}{\linewidth}{Xccccc}
    \toprule
        Cue &	Freq &	App. &	*	& Prod	& Cov \\
    \midrule
        (the, friend)	&	66040	&	4	&	2	&	0.5	&	0.004 \\
        (her, the)  	&	112344	&	8	&	5	&	0.625	&	0.008 \\
        (girl, the) 	&	60400	&	8	&	4	&	0.5	&	0.008 \\
        (the, woman)	&	66040	&	8	&	4	&	0.5	&	0.008 \\
        (on, the)   	&	94224	&	10	&	7	&	0.7	&	0.010 \\
        (of, the)   	&	103888	&	11	&	6	&	0.545	&	0.011 \\
        ('s, the)   	&	80936	&	11	&	6	&	0.545	&	0.011 \\
        (the, they) 	&	96520	&	12	&	6	&	0.5	&	0.012 \\
        (his, the)  	&	95432	&	14	&	8	&	0.571	&	0.014 \\
        (in, the)   	&	96640	&	15	&	6	&	0.4	&	0.015 \\
        (man, the)  	&	159456	&	16	&	8	&	0.5	&	0.016 \\
        (woman, the)	&	176368	&	16	&	8	&	0.5	&	0.016 \\
        (my, the)   	&	94224	&	17	&	7	&	0.412	&	0.017 \\
        (was, the)  	&	138920	&	17	&	7	&	0.412	&	0.017 \\
        (the, my)   	&	119380	&	20	&	10	&	0.5	&	0.020 \\
        (the, it)   	&	193040	&	22	&	11	&	0.5	&	0.022 \\
        (a, the)    	&	169120	&	22	&	10	&	0.455	&	0.022 \\
        (i, the)    	&	165496	&	28	&	16	&	0.571	&	0.028 \\
        (the, i)    	&	378460	&	28	&	13	&	0.464	&	0.028 \\
        (to, the)   	&	167912	&	30	&	14	&	0.467	&	0.030 \\
        (the, him)  	&	83820	&	30	&	15	&	0.5	&	0.030 \\
        (the, got)  	&	60960	&	34	&	17	&	0.5	&	0.034 \\
        (the, off)  	&	58420	&	38	&	19	&	0.5	&	0.038 \\
        (the, went) 	&	66040	&	38	&	19	&	0.5	&	0.038 \\
        (the, she)  	&	383540	&	38	&	19	&	0.5	&	0.038 \\
        (the, 's)   	&	78740	&	38	&	19	&	0.5	&	0.038 \\
        (the, from) 	&	71120	&	39	&	20	&	0.513	&	0.039 \\
        (the, out)  	&	58420	&	43	&	21	&	0.488	&	0.043 \\
        (the, he)   	&	393700	&	43	&	21	&	0.488	&	0.043 \\
        (the, her)  	&	373380	&	51	&	26	&	0.51	&	0.051 \\
        (the, his)  	&	243840	&	53	&	27	&	0.509	&	0.053 \\
        (the, of)   	&	86360	&	54	&	27	&	0.5	&	0.054 \\
        (the, with) 	&	86360	&	58	&	29	&	0.5	&	0.058 \\
        (the, for)  	&	86360	&	60	&	30	&	0.5	&	0.060 \\
        (the, in)   	&	160020	&	84	&	42	&	0.5	&	0.084 \\
        (the, on)   	&	139700	&	86	&	44	&	0.512	&	0.086 \\
        (the, was)  	&	332740	&	98	&	49	&	0.5	&	0.098 \\
        (the, the)  	&	1534160	&	145	&	73	&	0.503	&	0.145 \\
        (the, to)   	&	302260	&	152	&	75	&	0.493	&	0.152 \\
        (the, a)    	&	403860	&	194	&	98	&	0.505	&	0.194 \\

    \bottomrule
    \end{tabularx}
    \caption{Pairwise (a token from Premise + Alternative) annotation artifacts in balanced COPA.}
    \label{tab:copa-artifacts}
\end{table}

==> tables/all_single_que_annotation_artifacts.tex <==
\begin{table}[t]
    \centering
    \begin{tabularx}{\linewidth}{Xccccc}
    \toprule
        Cue     &	Freq &	App. &	*	&   Prod.	&   Cov. \\
    \midrule
        went	&	26	&	22	&	16	&	0.727	&	0.044 \\
        he	    &	155	&	22	&	10	&	0.455	&	0.044 \\
        i	    &	149	&	23	&	9	&	0.391	&	0.046 \\
        off	    &	23	&	23	&	12	&	0.522	&	0.046 \\
        out	    &	23	&	23	&	10	&	0.435	&	0.046 \\
        from	&	28	&	24	&	11	&	0.458	&	0.048 \\
        his	    &	96	&	27	&	8	&	0.296	&	0.054 \\
        her	    &	147	&	27	&	14	&	0.519	&	0.054 \\
        of	    &	34	&	28	&	15	&	0.536	&	0.056 \\
        for	    &	34	&	32	&	21	&	0.656	&	0.064 \\
        with	&	34	&	32	&	12	&	0.375	&	0.064 \\
        on	    &	55	&	45	&	18	&	0.400	&	0.090 \\
        in	    &	63	&	47	&	26	&	0.553	&	0.094 \\
        was	    &	131	&	55	&	34	&	0.618	&	0.110 \\
        to	    &	119	&	82	&	33	&	0.402	&	0.164 \\
        the	    &	604	&	85	&	33	&	0.388	&	0.170 \\
        a	    &	159	&	106	&	61	&	0.575	&	0.212 \\

    \bottomrule
    \end{tabularx}
    \caption{The most productive annotation artifacts in COPA.}
    \label{tab:copa-artifacts}
\end{table}

==> tables/table_balanced_easy_hard_evaluation.tex <==



%% DO NOT UPDATE



\begin{table*}[t]
    \centering
    \begin{tabular}{llccc}
    \toprule
        Model	&   Training data & Overall &   Easy    &   Hard \\
    \midrule
	 BERT-large-FT & B-COPA & 4.5 ($\pm$ 0.7) &  74.7 ($\pm$ 0.4) &  74.4 ($\pm$ 0.9) \\
	 BERT-large-FT & B-COPA (50\%) & 74.3 ($\pm$ 2.2) &  76.8 ($\pm$ 1.9) &  72.8 ($\pm$ 3.1) \\
	 BERT-large-FT & COPA	& 76.5 ($\pm$ 2.7) &  83.9 ($\pm$ 4.4) &  71.9 ($\pm$ 2.5) \\
    \bottomrule
    \end{tabular}
    \caption{Results of evaluation on Balanced COPA.
    \emph{Easy}: instances with superficial cues, \emph{Hard}: instances without superficial cues.}
    \label{tab:balanced-easy-hard-evaluation}
\end{table*}

==> tables/table_balanced_nonfinetuned.tex <==



%% DO NOT UPDATE



\begin{table*}[t]
    \centering
    \begin{tabular}{llccc}
    \toprule
        Model	&   Training data & Overall &   Easy    &   Hard \\
    \midrule
	 BERT-large & B-COPA	& 70.5 ($\pm$ 2.5) &  72.6 ($\pm$ 2.3) &  69.1 ($\pm$ 2.7) \\
	 BERT-large & B-COPA (50\%)	& 69.9 ($\pm$ 1.9) &  71.2 ($\pm$ 1.3) &  69.0 ($\pm$ 3.5) \\
	 BERT-large  & COPA	& 71.7 ($\pm$ 0.5) &  80.5 ($\pm$ 0.4) &  66.3 ($\pm$ 0.8) \\
    RoBERTa-lg-BC & B-COPA    &  76.7 ($\pm$ 0.8) &  73.3 ($\pm$ 1.5) &  78.8 ($\pm$ 2.0) \\
    RoBERTa-lg-BC0.5 & B-COPA (50\%) &  72.4 ($\pm$ 2.0) &  72.1 ($\pm$ 1.7) &  72.6 ($\pm$ 2.1) \\
    RoBERTa-lg & COPA       &  76.4 ($\pm$ 0.7) &  79.6 ($\pm$ 1.0) &  74.4 ($\pm$ 1.1) \\
	 \midrule
 	BERT-base-NSP	& None & \textbf{66.4}	& 66.2	& \textbf{66.7} \\
 	BERT-large-NSP	& None & 65.0	& \textbf{66.9}	& 62.1 \\
    \bottomrule
    \end{tabular}
    \caption{Results of non-fine-tuned models on Balanced COPA.
    \emph{Easy}: instances with superficial cues, \emph{Hard}: instances without superficial cues.}
    \label{tab:balanced-easy-hard-evaluation_nft}
\end{table*}

==> tables/table_premise_oblivious.tex <==
\begin{table}[t]
    \centering
    \begin{tabularx}{\linewidth}{Xccc}
    \toprule
        Model	    &   Max	    &   Mean    &	Stdev \\
    \midrule
      BERT-large-FT	&   0.610	&   0.606	&   0.003 \\
%      BERT-large	&   0.596	&   0.577	&   0.026 \\
    \bottomrule
    \end{tabularx}
    \caption{Performance of BERT on COPA test set.}
    \label{tab:premise-oblivious}
\end{table}

==> tables/table_sensitivity.tex <==
  \begin{table*}[t]
    \centering
    \begin{tabular}{llllll}
    \toprule
  Set	&	Model	&	Fine-tuning data & Non-spurious cue	&	Spurious cue	&	Sensitivity \\
    \midrule
  Test (Easy)	&	BERT-large	& None &	11.628 ($\pm$6.564)	&	7.761 ($\pm$5.714)	&	0.667 \\
  Test (Easy)	&	BERT-large-FT	& COPA &	14.247 ($\pm$6.779)	&	10.100 ($\pm$5.366)	&	0.709 \\
  Test (Easy)	&	BERT-large-FT	& B-COPA &	11.779 ($\pm$5.696)	&	7.789 ($\pm$4.810)	&	0.661 \\
  Test (Hard)	&	BERT-large	&	None & 11.245 ($\pm$6.528)	&	9.065 ($\pm$6.498)	&	0.806 \\
  Test (Hard)	&	BERT-large-FT	&	COPA & 13.621 ($\pm$6.033)	&	9.364 ($\pm$5.227)	&	0.687 \\
  Test (Hard)	&	BERT-large-FT	& B-COPA & 11.742 ($\pm$5.572)	&	7.345 ($\pm$4.603)	&	0.626 \\
  
      \bottomrule
    \end{tabular}
    \caption{Sensitivity to spurious cues.}
    \label{tab:sensitivity}
\end{table*}
